Toward Trustworthy Neural Program Synthesis

We develop an approach to estimate the probability that a program sampled from a large language model is correct. Given a natural language description of a programming problem, our method samples both candidate programs as well as candidate predicates specifying how the program should behave. This allows learning a model that forms a well-calibrated probabilistic prediction of program correctness. Our system also infers which predicates are useful to explain the behavior of the generated code, and humans preferred these in a human study over raw language model outputs. Our method is simple, easy to implement, and maintains state of the art generation accuracy results.

==> Prompts/HumanEval_spec_prompt.tex <==
\begin{Verbatim}[breaklines=true, breakanywhere=true]
# Problem 1

from typing import List

def filtered_even_integers(input_list: List[int]) -> List[int]:
    """ Given a list of integers, return a list that filters out the even integers.
    >>> filtered_even_integers([1, 2, 3, 4])
    [1, 3]
    >>> filtered_even_integers([5, 4, 3, 2, 1])
    [5, 3, 1]
    >>> filtered_even_integers([10, 18, 20])
    []
    """
    pass # To-do: implement

# Test 1

def test_filtered_even_integers(input_list: List[Int]):
    """ Given an input `input_list`, test whether the function `filtered_even_integers` is implemented correctly.
    """
    output_list = filtered_even_integers(input_list)
    # check if the output list only contains odd integers
    for integer in output_list:
        assert integer % 2 == 1
    # check if all the integers in the output list can be found in the input list
    for integer in output_list:
        assert integer in input_list

# run the testing function `test_filtered_even_integers` on a new testcase
test_filtered_even_integers([31, 24, 18, 99, 1000, 523, 901])

# Problem 2

def repeat_vowel(input_str: str) -> str:
    """ Return a string where the vowels (`a`, `e`, `i`, `o`, `u`, and their capital letters) are repeated twice in place.
    >>> repeat_vowel('abcdefg')
    'aabcdeefg'
    >>> repeat_vowel('Amy Emily Uber')
    'AAmy EEmiily UUbeer'
    """
    pass # To-do: implement

# Test 2

def test_repeat_vowel(input_str: str) :
    """ Given an input `input_str`, test whether the function `repeat_vowel` is implemented correctly.
    """
    output_str = repeat_vowel(input_str)
    vowels = ['a', 'A', 'e', 'E', 'i', 'I', 'o', 'O', 'u', 'U']
    # check if the number of vowels in the  output string is doubled
    # First get the number of vowels in the input
    number_of_vowels_input = sum([input_str.count(vowel) for vowel in vowels])
    # Then get the number of vowels in the output
    number_of_vowels_output = sum([output_str.count(vowel) for vowel in vowels])
    assert number_of_vowels_input * 2 == number_of_vowels_output

# run the testing function `test_repeat_vowel` on a new testcase
test_repeat_vowe('ABCDEabcdeABCDE YOUUOY')
\end{Verbatim}

==> Prompts/MBPP_spec_prompt.tex <==
\begin{Verbatim}[breaklines=true, breakanywhere=true]
# Problem 1

def filtered_even_integers(input_list: list) -> list:
    """
    Given a list of integers, return a list that filters out the even integers.
    """
    pass # To-do: implement

# Test 1

def test_filtered_even_integers(input_list: list):
    """
    Given an input `input_list`, test whether the function `filtered_even_integers` is implemented correctly.
    """
    output_list = filtered_even_integers(input_list)
    # check if the output list only contains odd integers
    for integer in output_list:
        assert integer % 2 == 1
    # check if all the integers in the output list can be found in the input list
    for integer in output_list:
        assert integer in input_list

# run the testing function `test_filtered_even_integers` on a new testcase
test_filtered_even_integers([31, 24, 18, 99, 1000, 523, 901])

# Problem 2

def repeat_vowel(input_str: str) -> str:
    """
    Return a string where the vowels (`a`, `e`, `i`, `o`, `u`, and their capital letters) are repeated twice in place
    """
    pass # To-do: implement

# Test 2

def test_repeat_vowel(input_str: str):
    """
    Given an input `input_str`, test whether the function `repeat_vowel` is implemented correctly.
    """
    output_str = repeat_vowel(input_str)
    vowels = ['a', 'A', 'e', 'E', 'i', 'I', 'o', 'O', 'u', 'U']
    # check if the number of vowels in the  output string is doubled
    # First get the number of vowels in the input
    number_of_vowels_input = sum([input_str.count(vowel) for vowel in vowels])
    # Then get the number of vowels in the output
    number_of_vowels_output = sum([output_str.count(vowel) for vowel in vowels])
    assert number_of_vowels_input * 2 == number_of_vowels_output

# run the testing function `test_repeat_vowel` on a new testcase
test_repeat_vowe('ABCDEabcdeABCDE YOUUOY')
\end{Verbatim}


==> figure2_prompt_example.tex <==
\definecolor{titlebox}{RGB}{36, 151, 190}
\definecolor{completion-color}{RGB}{30, 70, 240}
\definecolor{light-gray}{gray}{1}
\definecolor{lstbackground}{gray}{0}
\definecolor{mygray}{gray}{0.85}
%\definecolor{completion-color}{gray}{0.6}
\lstset{
  basicstyle=\footnotesize\ttfamily,
  %columns=fullflexible,
  %keepspaces=true,
  numbers=none,
  %breaklines=false,
  backgroundcolor=\color{light-gray}
%   backgroundcolor=titlebox
}

\lstset{escapeinside={<@}{@>}}

\newtcolorbox{BlueBox}[2][]{
    top = 0.1mm,
    bottom = 0.1mm,
    left = 0.1mm,
    right = 0.1mm,
                lower separated=false,
                colback=white,
                frame hidden,
colframe=black,fonttitle=\bfseries,
borderline={1pt}{0pt}{mygray},
colbacktitle=mygray,
coltitle=black,
enhanced,
attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
                 boxed title style={boxrule=0pt,colframe=white,},
title=#2,#1}
\newtcolorbox{BlueBox2}[2][]{%
    enhanced,
    top = 0.1mm,
    bottom = 0.1mm,
    left = 0.1mm,
    right = 0.1mm,
    colback   = light-gray,
    colframe  = blue!30!black, 
    arc       = 0mm, 
    %outer arc = 1mm, 
    fonttitle = \Large\textbf,
    center title, 
    title     = #2,
    #1}
  
\begin{figure*}[h]
\begin{adjustbox}{width=\textwidth,center}
\begin{tcbraster}[raster width=22.5cm, raster columns=2,raster valign=top]%<------------added
\begin{BlueBox}[bottom=2mm]{Generating Programs}
\begin{lstlisting}
def sub_list(nums1 : list, nums2 : list) -> list:
    """
    Write a function to subtract two lists element-wise.
    """
    <@\color{completion-color}return list(map(lambda x, y: x-y, nums1, nums2))@>
\end{lstlisting} 
\end{BlueBox}
\begin{BlueBox}[bottom=-2mm]{Generating Input-Output Specifications}
\begin{lstlisting}
def sub_list(nums1 : list, nums2 : list) -> list:
    """
    Write a function to subtract two lists element-wise.
    """
    pass # To-do: implement
# Check if sub_list works
assert sub_list(<@\color{completion-color}[2, 3, 1], [1, 1, 1]) == [1, 2, 0])@>
\end{lstlisting}
\end{BlueBox}
\end{tcbraster}
\end{adjustbox}

\vspace{-4.5mm}
\begin{adjustbox}{width=14cm,center}
\begin{tcbraster}[raster width=20cm, raster columns=1, raster valign=top]
\begin{BlueBox}{Generating Logical-Relation Specifications}
\begin{lstlisting}
<@\textit{[Two-Shot Examples]}@>
<@\vspace{-0.5cm}@>
<@\hspace{1.5cm} \textit{\vdots}@>
# Problem 3
# Write a function to subtract two lists element-wise.
def sub_list(nums1,nums2):
    pass # To-do: implement
# Test 3    
<@\color{completion-color}def test\_sub\_list(nums1 : list, nums2 : list):@>
    <@\color{completion-color}"""@>
    <@\color{completion-color}Given two lists `nums1` and `nums2`, test whether function `sub\_list` is implemented correctly.@>
    <@\color{completion-color}"""@>
    <@\color{completion-color}output\_list = sub\_list(nums1, nums2)@>
    <@\color{completion-color}\# check if the length of the output list is the same as the lengths of the input lists@>
    <@\color{completion-color}assert len(output\_list) == len(nums1) == len(nums2)@>
    <@\color{completion-color}\# check if the output list has the expected elements@>
    <@\color{completion-color}for i in range(len(output\_list)):@>
        <@\color{completion-color}assert output\_list[i] == nums1[i] - nums2[i]@>

<@\color{completion-color}\# run the testing function `test\_sub\_list` on a new testcase@>
<@\color{completion-color}test\_sub\_list([1, 2, 3, 4], [10, 9, 8, 7])@>

\end{lstlisting}
\end{BlueBox}
\end{tcbraster}
\end{adjustbox}
\caption{Our systems uses different prompts to generate programs, input-output tests, and logical relations. Here we also show the example completion from the model in blue.}\label{fig:prompting}
\end{figure*}


==> figure2_prompt_example_table.tex <==

\definecolor{light-gray}{gray}{0.97}
\definecolor{completion-color}{gray}{0.75}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  keepspaces=true,
  numbers=none,
  backgroundcolor=\color{light-gray}
}

  
  
\lstset{escapeinside={<@}{@>}}

\mdfdefinestyle{MyFrame}{
  %linecolor=black,
  hidealllines=true,
  backgroundcolor=light-gray,
  innerleftmargin=6pt,
  innertopmargin=0pt,
  innerbottommargin=0pt}
  
\begin{figure}
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{p{16cm} p{16cm}}
%\multicolumn{2}{cc}{Generating Programs & Generating IO Tests}\\[-10pt]
\begin{mdframed}[style=MyFrame,nobreak=true]
\begin{lstlisting}
def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    <@\color{completion-color}return list(filter(lambda x: isinstance(x, int), values)) @>
\end{lstlisting} 
\end{mdframed}&
%\multicolumn{1}{c}{Generating IO Tests}\\[-10pt]
\begin{mdframed}[style=MyFrame,nobreak=true]
\begin{lstlisting}
def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    pass # To-do: implement

# Check if filter_integers works
assert filter_integers(<@\color{completion-color}filter\_integers(['a', 1, 2, 3]) == [1, 2, 3]@>
\end{lstlisting}
\end{mdframed}\\
\multicolumn{2}{c}{Generating Specification Tests}\\[-10pt]
\begin{mdframed}[style=MyFrame,nobreak=true]
\begin{lstlisting}
<@\textit{[Few-Shot Examples]}@>
<@\vspace{-0.5cm}@>
<@\hspace{1.5cm} \textit{\vdots}@>
# Problem 3

def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    # TODO
    pass
    
# Test 3    

def test_filter_integers(values: List[Any]):
    """ Given an input `values`, test whether the function `filter_integers` is implemented correctly. """
    output_list = filter_integers(values)
<@\color{completion-color}    \# check if only integers are in the output@>
<@\color{completion-color}    for value in output\_list:@>
<@\color{completion-color}        assert type(value) == int@>
<@\color{completion-color}    \# check if all the integers in the output can be found in the input@>
<@\color{completion-color}    for value in output\_list:@>
<@\color{completion-color}        assert value in values@>

<@\color{completion-color}\# run the testing function `test\_filter\_integers` on a new testcase@>
<@\color{completion-color}test\_filter\_integers(['a', 1, 'b', 2, 3, 'c'])@>
\end{lstlisting}
\end{mdframed}
\end{tabular}
\end{adjustbox}
\caption{This figure should show the initial prompt, sampled programs, how the prompt is transformed to generate test cases, and sampled test cases}\label{fig:prompting}
\end{figure}


==> figure2_prompt_humaneval_example.tex <==
\definecolor{titlebox}{RGB}{36, 151, 190}
\definecolor{completion-color}{RGB}{36, 161, 210}
\definecolor{light-gray}{gray}{1}
\definecolor{lstbackground}{gray}{0}
%\definecolor{completion-color}{gray}{0.6}
\lstset{
  basicstyle=\footnotesize\ttfamily,
  %columns=fullflexible,
  %keepspaces=true,
  numbers=none,
  %breaklines=false,
  backgroundcolor=\color{light-gray}
%   backgroundcolor=titlebox
}

\lstset{escapeinside={<@}{@>}}

\newtcolorbox{BlueBox}[2][]{
    top = 0.1mm,
    bottom = 0.1mm,
    left = 0.1mm,
    right = 0.1mm,
                lower separated=false,
                colback=white,
colframe=black,fonttitle=\bfseries,
colbacktitle=titlebox,
coltitle=white,
enhanced,
attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
                 boxed title style={boxrule=0pt,colframe=white,},
title=#2,#1}
\newtcolorbox{BlueBox2}[2][]{%
    enhanced,
    top = 0.1mm,
    bottom = 0.1mm,
    left = 0.1mm,
    right = 0.1mm,
    colback   = light-gray,
    colframe  = blue!30!black, 
    arc       = 0mm, 
    %outer arc = 1mm, 
    fonttitle = \Large\textbf,
    center title, 
    title     = #2,
    #1}
  
\begin{figure}
\begin{adjustbox}{width=14cm,center}
\begin{tcbraster}[raster width=27cm, raster columns=2,raster valign=top]%<------------added
\begin{BlueBox}[bottom=7mm]{Generating Programs}
\begin{lstlisting}
def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    <@\color{completion-color}return list(filter(lambda x: isinstance(x, int), values)) @>
\end{lstlisting} 
\end{BlueBox}
\begin{BlueBox}{Generating Input-Output Specifications}
\begin{lstlisting}
def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    pass # To-do: implement

# Check if filter_integers works
assert filter_integers(<@\color{completion-color}['a', 1, 2, 3]) == [1, 2, 3]@>
\end{lstlisting}
\end{BlueBox}
\end{tcbraster}
\end{adjustbox}

\vspace{-3.5mm}
\begin{adjustbox}{width=14cm,center}
\begin{tcbraster}[raster width=24cm, raster columns=1, raster valign=top]
\begin{BlueBox}{Generating Logical-Relation Specifications}
\begin{lstlisting}
<@\textit{[Two-Shot Examples]}@>
<@\vspace{-0.5cm}@>
<@\hspace{1.5cm} \textit{\vdots}@>
# Problem 3

def filter_integers(values: List[Any]) -> List[int]:}
    """ Filter given list of any python values only for integers
    >>> filter_integers(['a', 3.14, 5])
    [5]
    >>> filter_integers([1, 2, 3, 'abc', {}, []])
    [1, 2, 3]
    """
    # TODO
    pass
    
# Test 3    

<@\color{completion-color}def test\_filter\_integers(values: List[Any]):@>
<@\color{completion-color}    """ Given an input `values`, test whether the function `filter\_integers` is implemented correctly. """@>
<@\color{completion-color}    output\_list = filter\_integers(values)@>
<@\color{completion-color}    \# check if only integers are in the output@>
<@\color{completion-color}    for value in output\_list:@>
<@\color{completion-color}        assert type(value) == int@>
<@\color{completion-color}    \# check if all the integers in the output can be found in the input@>
<@\color{completion-color}    for value in output\_list:@>
<@\color{completion-color}        assert value in values@>

<@\color{completion-color}\# run the testing function `test\_filter\_integers` on a new testcase@>
<@\color{completion-color}test\_filter\_integers(['a', 1, 'b', 2, 3, 'c'])@>
\end{lstlisting}
\end{BlueBox}
\end{tcbraster}
\end{adjustbox}
\caption{Our systems utilizes different prompts to generate programs, input-output tests, and specification. Here we also show the example completion from the model in gray.}\label{fig:prompting}
\end{figure}

